To Reverse the Gradient or Not: An Empirical Comparison of Adversarial and Multi-task Learning in Speech Recognition

Transcribed datasets typically contain speaker identity for each instance in the data. We investigate two ways to incorporate this information during training: Multi-Task Learning and Adversarial Learning. In multi-task learning, the goal is speaker prediction; we expect a performance improvement with this joint training if the two tasks of speech recognition and speaker recognition share a common set of underlying features. In contrast, adversarial learning is a means to learn representations invariant to the speaker. We then expect better performance if this learnt invariance helps generalizing to new speakers. While the two approaches seem natural in the context of speech recognition, they are incompatible because they correspond to opposite gradients back-propagated to the model. In order to better understand the effect of these approaches in terms of error rates, we compare both strategies in controlled settings. Moreover, we explore the use of additional untranscribed data in a semi-supervised, adversarial learning manner to improve error rates. Our results show that deep models trained on big datasets already develop invariant representations to speakers without any auxiliary loss. When considering adversarial learning and multi-task learning, the impact on the acoustic model seems minor. However, models trained in a semi-supervised manner can improve error-rates.

==> 02_relatedwork.tex <==
% !TEX root =  main.tex
\section{Introduction}
%A major difficulty of speech recognition comes from speaker differences in intonation and delivery. Luckily, most datasets come with speaker identity labels. In this work we look into leveraging them in a single pass as the acoustic model training.

The minimal components of a speech recognition dataset are audio recordings and their corresponding transcription. They also typically contain an additional information, which is the identity label of the speaker corresponding to each utterance. As speaker variations are one of the most challenging aspects of speech data, this information can be leveraged to improve the performance and robustness of speech recognition systems.

In this work we focus on the task of end-to-end speech recognition. In this setting, we are given audio recordings and their transcripts, and train a neural network to output letters with a sequence-based criterion. During training, we also have access to the identity of the speaker of each utterance. Senior \& Lopez-Moreno \cite{ivector_input1}, and Peddinti et al. \cite{ivector_input2} have used speaker information and derived features as an additional input to the acoustic model. We study how to best exploit these labels, and systematically compare two approaches that have been proposed, yet are intrinsically incompatible: multi-task learning, and adversarial learning.

Multi-task learning \cite{caruana1998multitask, ronan_language} for speech recognition is a training scheme based on the assumption that performances on the task of interest can be improved by jointly training with auxiliary tasks. Previous work has explored using auxiliary tasks such as gender or context \cite{mtl_overview}, as well as speaker classification \cite{mtl_speaker}. 
%In the latter, this means that minimizing the classification error on a speaker identification task additionally to the transcription loss can yield better transcriptions. 
In the context of end-to-end speech recognition, a way of performing multi-task learning is to add a speaker classification branch in parallel of the main branch trained for transcription. All layers below the fork of the two branches are thus trained for both speech recognition and speaker classification.

An opposite approach is to assume that good acoustic representations should be invariant to any task that is not the speech recognition task, in particular the speaker characteristics. A method to learn %recent line of work \cite{domain_adversarial_nn} proposes a method to learn 
such invariances is adversarial training \cite{domain_adversarial_nn}: the branch of the speaker classification task is trained to reduce its classification error, however the layers below the fork in the main branch are trained to maximize the loss of this speaker classifier. By doing so, they learn invariance to speaker characteristics. This approach has been previously used for speech recognition to learn invariance to noise conditions \cite{adversarial_noise} and speaker identity \cite{adversarial_speaker}.

Our study arises from two observations. First, both the multi-task and adversarial approaches described above have been used with the same purpose despite being fundamentally opposed, and this raises the question of which one is the most appropriate choice to improve the performance of speech recognition systems. Secondly, they only differ by a simple computational step which consists in reversing the gradient at the fork between the speaker branch and the main branch to switch from multi-task learning to adversarial. This allows for controlled experiments where both approaches can be compared with equivalent architectures and number of parameters.

In this work, we perform a systematic comparison between multi-task and adversarial training for the task of large vocabulary speech recognition on the Wall Street Journal dataset (WSJ) \cite{wsj}. Knowing whether the speaker information should be used to impact low level or high level representations is also a valuable information, so for each approach we experiment with three levels to fork the speaker branch to: lower layer, middle and upper layer. On the full WSJ dataset, we show that both multi-task and adversarial training approaches improve on an equivalent architecture that does not use speaker information. We also perform speaker classification on the trained models and show that models trained in multi-task produce representations that are discriminative for speaker, while models trained in an adversarial setting learn some level of invariance. We then explore unbalanced subsets of WSJ, where we have access to many utterances of a few speakers, or the opposite.




==> 05_spkclass.tex <==
\section{Encoded Speaker Information}
While training an acoustic model usually we do not use any information about the speaker. Since we would like to use speaker labels as another supervision to network we would like to assess \emph{to what extent the network encodes the speaker identity?} The motivation for answering this question is two folded (i) to analyze the networks' behaviour with respect to the speaker information, (ii) the main idea beyond speaker adversarial training is to generate representation which will be speaker invariant, having a measurement for the amount of speaker information encoded in the representation can give us an intuitive assessment of how further can we improve results using the above approach.

To tackle this question, we follow a similar approach to the one proposed in \cite{adi2016fine, adi2017analysis}, first train an acoustic model on WSJ dataset.  (later on we will consider this model as the speaker branch).

first we train an acoustic model without speaker labels, denoted as our baseline. Then, we extract representations of the speech signal from different layers in the model and train a classifier to classify the speaker based on the models' representation. After training we measure the classifier's accuracy, convergence speed, etc. and use it to analyze the presence of speaker identity in the representation.

The basic premise of this approach is that if we cannot train a classifier to predict this basic property based on its representation from the model, then this property is not encoded in the representation, or rather, not encoded in a useful way, considered the way it will be used. To make things clear, we are not interested in improving speaker classification results but rather to have a comparison between the models based on the classifier's performance.

Our classification model is the same as the speaker branch, it is composed of two gated convolutional layers with a weight normalization layer, and we train each speaker model for 10 epochs. 

With conducted the above experiment for the full WSJ dataset, $\minspk$ and $\maxspk$, using representations from $\inlayer, \midlayer$ and $\outlayer$. Figure~\ref{fig:spkclass}, presents the classification results of all models. Results suggest that all three models already develop a speaker invariant representation as we go deeper in the network. Those results provide us with more information on how much we can improve using adversarial training or multi-task training techniques.

\begin{figure} [h!]
  \includegraphics[width=\linewidth]{img/spk-acc.png}
  \caption{Speaker classification accuracy using the representation from different layers of the network. Results are reported for three different settings, i.e. Full dataset, $\minspk$ and $\maxspk$, using three different layers in the network, i.e. $\inlayer$, $\midlayer$, $\outlayer$}
  \label{fig:spkclass}
\end{figure}


==> 06_futurework.tex <==
% !TEX root =  main.tex
%\vspace{-0.1cm}
\section{Future Work}
%We conducted a controlled comparison between speaker AL and speaker MT for automatic speech recognition on WSJ dataset. 
%We used three different settings for both methods, together with semi-supervised settings. In addition, we analyzed the amount of speaker information already embedded in the network. Results suggests that both methods can improve LER over the baseline, however when considering WER things are ambiguous. 

For future work, we would like further inspect and analyze the integration between acoustic models and language models and train them jointly. Additionally, we would like to explore the effect of adversarial learning and adversarial semi-supervised learning for small datasets and low-resource languages.

